FedBN: Federated Learning on Non-IID Features via Local Batch Normalization

The emerging paradigm of federated learning (FL) strives to enable collaborative training of deep models on the network edge without centrally aggregating raw data and hence improving data privacy. In most cases, the assumption of independent and identically distributed samples across local clients does not hold for federated learning setups. Under this setting, neural network training performance may vary significantly according to the data distribution and even hurt training convergence. Most of the previous work has focused on a difference in the distribution of labels or client shifts. Unlike those settings, we address an important problem of FL, e.g., different scanners/sensors in medical imaging, different scenery distribution in autonomous driving (highway vs. city), where local clients store examples with different distributions compared to other clients, which we denote as feature shift non-iid. In this work, we propose an effective method that uses local batch normalization to alleviate the feature shift before averaging models. The resulting scheme, called FedBN, outperforms both classical FedAvg, as well as the state-of-the-art for non-iid data (FedProx) on our extensive experiments. These empirical results are supported by a convergence analysis that shows in a simplified setting that FedBN has a faster convergence rate than FedAvg. Code is available at https://github.com/med-air/FedBN.

==> Federated Learning for Non-IID Data/abstract.tex <==
The emerging paradigm of federated learning (FL) strives to enable collaborative training of deep models on the network edge without centrally aggregating raw data and hence improving data privacy. In most cases, the assumption of independent and identically distributed samples across local clients does not hold for federated learning setups. Under this setting, neural network training performance may vary significantly according to the data distribution and even hurt training convergence. Most of the previous work has focused on a difference in the distribution of labels or client shifts. Unlike those settings, we address an important problem of FL, e.g., different scanners/sensors in medical imaging, different scenery distribution in autonomous driving (highway vs. city), where local clients store examples with different distributions compared to other clients, which we denote as \textit{feature shift non-iid}. In this work, we propose an effective method that uses local batch normalization to alleviate the feature shift before averaging models. The resulting scheme, called \textit{FedBN}, outperforms both classical FedAvg, as well as the state-of-the-art for non-iid data (FedProx) on our extensive experiments. These empirical results are supported by a convergence analysis that shows in a simplified setting that FedBN has a faster convergence rate than FedAvg. Code is available at \href{https://github.com/med-air/FedBN}{https://github.com/med-air/FedBN}.





==> Federated Learning for Non-IID Data/conclution.tex <==
\vspace{-3mm}
\section{Conclusion and Discussion}
This work proposes a novel federated learning aggregation method called FedBN that keeps the local Batch Normalization parameters not synchronized with the global model, such that it mitigates feature shifts in non-IID data.  We provide convergence guarantees for FedBN in realistic federated settings under the overparameterized neural networks regime, while also accounting for practical issues. In our experiments, our evaluation across a suite of federated datasets has demonstrated that FedBN can significantly improve the convergence behavior and model performance of non-IID datasets. We also demonstrate the effectiveness of FedBN in scenarios that where a new client with an unknown domain joins the FL system (see Appendix~\ref{app:test}).

FedBN is independent of the communication and aggregation strategy and thus can in practice be readily combined with different optimization algorithms, communication schemes, and aggregation techniques. The theoretical analysis of such combinations is an interesting direction for future work.

We also note that since FedBN makes only lightweight modifications to FedAvg and has much flexibility to be combined with other strategies, these merits allow us to easily integrate FedBN into existing tool-kits/systems, such as Pysyft \citep{ryffel2018generic}, Google TFF \citep{google}, Flower~\citep{beutel2020flower}, dlplatform~\citep{dlplatform} and FedML \citep{he2020fedml}\footnote{The implementations on \href{https://github.com/chairiq/dlplatforms}{dlplatform} and \href{https://github.com/adap/flower/tree/main/examples/pytorch_from_centralized_to_federated}{Flower} are available, and the implementation on \href{https://github.com/FedML-AI/FedML}{FedML} is to appear soon.}.

We believe that FedBN can improve a wide range of applications such as healthcare~\citep{rieke2020future} and autonomous driving~\citep{kamp2018efficient}. 
A few interesting directions for future work include analyzing what types of differences in local data can benefit from FedBN and explore the limits of FedBN. Moreover, privacy is an essential concern in FL. Invisible BN parameters in FedBN should make attacks on local data more challenging. It would be interesting to quantify the privacy-preservation improvement in FedBN.



==> Federated Learning for Non-IID Data/experiment.tex <==
\section{Experiments}
\label{sec:experiment}

In this section, we demonstrate that using local BN parameters is beneficial in the presence of feature shift across clients with heterogeneity data. Our novel local parameter sharing strategy, FedBN, achieves more robust and faster convergence for feature shift non-iid datasets and obtains better model performance compared to alternative methods. This is shown on both benchmark and large real-world datasets.

\iffalse
\subsection{Synthetic Data} %
\textbf{Settings.} We generate data from two-pair of multi-Gaussian distributions. For one pair, samples $(x,0)$ and $(x,1)$ are sampled from ${\cal N}(-1,~\Sigma_1)$ and ${\cal N}(1,~\Sigma_1)$ respectively, with coveriance $\Sigma_1 \in \R^{10 \times 10}$. For another pair, samples $(\Tilde{x},0)$ and $(\Tilde{x},1)$ are sampled from ${\cal N}(-1,~\Sigma_2)$ and ${\cal N}(1,~\Sigma_2)$ respectively, with coveriance $\Sigma_2 \in \R^{10 \times 10}$. Specifically, we design convariance matrix $\Sigma_1$ as an identity diagonal matrix and $\Sigma_2$ is different from $\Sigma_1$ by having non-zero values on off-diagonal entries. We train a two-layer neural network with 100 hidden neurons for 600 steps using cross-entropy loss and SGD optimizer with $1\times 10^{-5}$ learning rate. Denote $W_k$ and $b_k$ are the in-connection weigths and bias term of neuron $k$. We initialize the model parameters with $W_k \sim {\cal N}(0,\alpha^2\mathbf{I}),~b_k\sim{\cal N}(0,\alpha^2)$, where $\alpha = 10$.

\textbf{Results.} The aim of synthetic experiments is to study the behavior of using FedBN with a controlled setup. We achieve averaged $~100\%,~100\%$ on binary classification for FedAvg and FedBN. Figure~\ref{fig:converge rate} shows comparison of training loss curve over steps using FedAvg and FedBN, presenting that FedBN obtains significantly faster and more stable convergence relative to FedAvg.
\fi
%


\subsection{Benchmark Experiments}
\label{sec:benchmar_exp}
\paragraph{Settings:} We perform an extensive empirical analysis using a benchmark digits classification task containing different data sources with feature shift where each dataset is from a different domain. Data of different domains have heterogeneous appearance but share the same labels and label distribution.  Specifically, we use the following five datasets: SVHN \cite{netzer2011svhn}, USPS \cite{hull1994usps}, SynthDigits \cite{ganin2015synth&mnistm}, MNIST-M \cite{ganin2015synth&mnistm} and MNIST \cite{lecun1998mnist}. To match the setup in Section \ref{sec:method}, 
we truncate the sample size of the five datasets to their smallest number with random sampling, resulting in 7438 training samples in each dataset \footnote{\revision{This data preprocessing intends to strictly control non-related factors (e.g., imbalanced sample numbers across clients), so that the experimental findings can more clearly reflect the effect of local BN. Results without truncating are reported in Appendix~\ref{app:unequal}.}}.
Testing samples are held out and kept the same for all the experiments on this benchmark dataset.
Our classification model is a convolutional neural network where BN layers are added following each feature extraction layer (i.e., both convolutional and fully-connected). The architecture is detailed in Appendix~\ref{sec:benchmark_settings}. 

For model training, we use the cross-entropy loss and SGD optimizer with a learning rate of $10^{-2}$. If not specified, our default setting for local update epochs is $E=1$, and the default setting for the amount of data at each client is $10\%$ \footnote{\revision{Choosing 10\% fraction as default is based on (i) considering it as a typical setting to present general efficacy of our method; (ii) matching literature where the client size is usually around $100$ to $1000$ data points \citep{mcmahan2017communication,li2019convergence,hsu2019measuring}, which is a similar scale with respect to our 10\% setting (in terms of the absolute value of sample numbers).} 
} of the dataset original size. 
For the default non-iid setting, the FL system contains five clients. Each client exclusively owns data sampled from one of the five datasets.
More details are listed in Appendix~\ref{sec:benchmark_settings}.  
\begin{figure}[t]
    \centering
    \includegraphics[trim={0 100 0 160}, clip, scale=0.5]{converge_loss_removesimulation.pdf}
    \vspace{-6mm}
    \caption{
    Convergence of the training loss of FedBN and FedAvg on the digits classification datasets. FedBN exhibits faster and more robust convergence.}
    \label{fig:converge rate}
\end{figure}


\paragraph{Overviews:} In the following paragraphs, we present a comprehensive investigation on the properties of the proposed FedBN approach, including: (1) convergence rate; (2) behavior with respect to the choices of local update epochs; (3) performance on various amounts of data at each client; (4) effects at different level of heterogeneity; (5) %demonstrating dominance of FedBN 
comparison to state of the art (FedProx \citep{li2018federated}), and two baselines (FedAvg and SingleSet, i.e., training an individual model within each client). In Appendix~\ref{app:test}, we also provide empirical results for including a new client with data from an unknown domain into the learning system.% on the benchmark datasets.

\paragraph{Convergence Rate:} 
We analyze the training loss curve of FedBN in comparison with FedAvg, as shown in Fig. \ref{fig:converge rate}. The loss of FedBN goes down faster and smoother than FedAvg, indicating that FedBN has a larger convergence rate. Moreover, compared to FedAvg, FedBN presents smoother and more stable loss curves during learning. 
These experimental observations show consensus with what given by Corollary \ref{co:46}.
In addition, we present a more comprehensive comparison with different local update epochs $E$ on convergence rate of FedBN and FedAvg (see Appendix~\ref{sec:moreconv}). The results show similar patterns as in Fig~\ref{fig:converge rate}.
\vspace{-3mm}
\paragraph{Analysis of Local Updating Epochs:}
Aggregating at different frequencies may affect the learning behaviour. Although our theory and the default setting for the other experiment takes $E=1$, we demonstrate FedBN is effective for cases when $E>1$. In Fig.\ref{fig:scalability+digits_sota} (a), we explore $E = 1, 4, 8, 16$ and compare FedBN to baseline FedAvg.
As expected, an inverse relationship between the local updating epochs $E$ and testing accuracy implied for both FedBN and FedAvg shown in Fig.\ref{fig:scalability+digits_sota} (a). 
Zooming into the final testing accuracy, FedBN's accuracy stably exceeds the  accuracy  of FedAvg on various $E$ . 


\begin{figure*}[!t]
    \includegraphics[trim={0 80 0 105},clip,width=0.99\textwidth]{fig4_zerograd.pdf}
    \vspace{-2mm}
    \caption{Analytical experimental results on: (a) Analysis on different local updating epochs. FedBN consistently outperforms FedAvg in testing accuracy. (b) Model performance over varying dataset size on local clients.
    (c) Testing accuracy on different levels of heterogeneity.
    }
    \label{fig:scalability+digits_sota}
\end{figure*}




\paragraph{Analysis of Local Dataset Size:}
We vary the data amount for each client from $100\%$ to $1\%$ of its original dataset size, in order to observe FedBN behaviour over different data capacities at each client.
The results in Fig.\ref{fig:scalability+digits_sota} (b) present the accuracy of FedBN and SingleSet \footnote{\revision{Detailed statistics and FedAvg results are presented in Appendix \ref{app:4b}.}}. 
Testing accuracy starts to significantly drop when each of the local client is only attributed 20\% percentage of data from its original data amount. The improvement margin gained from FedBN increases as local dataset sizes decrease. The results indicate that FedBN can effectively benefit from collaborative training on distributed data, especially when each client only holds a small amount of data which are non-iid. 
\vspace{-3mm}


\paragraph{Effects of Statistical Heterogeneity:}
A salient question that arises is: to what degree of heterogeneity on feature shift FedBN is superior to FedAvg. To answer the question, we simulate a federated settings with varying heterogeneity as described below. We parcel each dataset into 10 subsets, one for each clients, with equal number of data samples and the same label distribution. We treat the clients generated from the same dataset as iid clients, while the clients generated from different datasets as non-iid clients. 

We start with including one client from each dataset in FL system. \revision{Then, we simultaneously add one client from each datasets while keep the existing clients $n$ times, for $n \in \{1,\dots,9\}$\footnote{\revision{Namely, each increment contains five non-iid clients.}} . For each setting, we train models from scratch.}
More clients correspond to less heterogenity. We show the testing accuracy under different level of heterogeneity in Fig.~\ref{fig:scalability+digits_sota} (c) and include a comparison with FedAvg, which is designed for iid FL. Our FedBN achieves substantially higher testing accuracy than FedAvg over all levels of heterogeneity.

\begin{wrapfigure}{r}{0.62\textwidth}
  \begin{center}
    \includegraphics[width=0.62\textwidth]{digits_sota_zero_grad.pdf}
  \end{center}
  \vspace{-3mm}
  \caption{Performance on benchmark experiments}
  \label{fig:compare}
\end{wrapfigure} 

\paragraph{Comparison with State-of-the-art:} To further validate our method, we compare FedBN with one of the current state-of-the-art methods for non-iid FL, FedProx \cite{li2018federated}, which also shares the benefit of easy adaptation to current FL frameworks in practice. We also include training on SingleSet and FedAvg as baselines. For each strategy, we split an independent testing datasets on clients and report the accuracy on the testing datasets. We perform 5-trial repeating experiment with different random seeds. The mean and standard deviation of the accuracy on each dataset over trials are shown in Fig.~\ref{fig:compare}\footnote{ \revision{Detailed statistics are shown in Appendix \ref{ap:figcompare}}}. From the results, we can make the following observation: (1) FedBN achieves the highest accuracy, consistently outperforming the state-of-the-art and baseline methods;
(2) FedBN achieves the most significant improvements on SVHN whose image appearance is very different from others (i.e., presenting more obvious feature shift); (3) FedBN shows a smaller variance in error over multiple runs, indicating its stability. 


\subsection{Experiments on real-world datasets}
To better understand how our proposed algorithm can be beneficial in real-word feature-shift non-iid, we have extensively validated the effectiveness of FedBN in comparison with other methods on three real-world datasets: image classification on Office-Caltech10~\citep{gong2012geodesic} with images acquired in different cameras or environments; image classification on DomainNet~\citep{peng2019moment} with different image styles; and a neurodisorder diagnosis task on ABIDE I \citep{di2014autism} with patients from different medical institutions\footnote{More details about the datasets and training process are listed in the Appendix~\ref{sec:real-world-settins} and \ref{sec:appabide}}.

\begin{table}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cccc|cccccc|cccc}
% \hline
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{4}{c|}{Caltech-10} & \multicolumn{6}{c}{DomainNet} &\multicolumn{4}{c}{ABIDE (medical)} \\ \cline{2-15} 
\multicolumn{1}{c|}{} & A & C & D & W  & C & I & P & Q & R & S & NYU & USM & UM & UCLA\\ \midrule
{\multirow{2}{*}{SingleSet}} &54.9&40.2&78.7&86.4 & 41.0 & 23.8 & 36.2 & \textbf{73.1} & 48.5& 34.0  &58.0 & 73.4& 64.3& 57.3\\
 \multicolumn{1}{c|}{}      &(1.5)&(1.6)&(1.3)&(2.4) &(0.9)&(1.2)&(2.7)&\textbf{(0.9)}&(1.9)&(1.1) &(3.3)&(2.2)&(1.4)&(2.4)\\
 \hline
\multirow{2}{*}{FedAvg} &54.1& 44.8& 66.9& 85.1   & 48.8 & 24.9 & 36.5 & 56.1 & 46.3 & 36.6 &62.7& 73.1& \textbf{70.7}& 64.7\\
\multicolumn{1}{c|}{} & (1.1)&(1.0)&(1.5)&(2.9) &(1.9)&(0.7)&(1.1)&(1.6)&(1.4)&(2.5)&(1.7)&(2.4)&\textbf{(0.5)}&(0.7)\\
\hline
\multirow{2}{*}{FedProx} &54.2& 44.5& 65.0 & 84.4  & 48.9 & 24.9 & 36.6 & 54.4 & 47.8 & 36.9 & 63.3& 73.0& 70.5& 64.5\\
\multicolumn{1}{c|}{} &(2.5)&(0.5)&(3.6)&(1.7) &(0.8)&(1.0)&(1.8)&(3.1)&(0.8)&(2.1) &(1.0)&(1.8)&(1.1)&(1.2)\\
\hline
\multirow{2}{*}{FedBN} &\textbf{63.0}& \textbf{45.3}& \textbf{83.1}& \textbf{90.5}   & \textbf{51.2} & \textbf{26.8} & \textbf{41.5} & 71.3& \textbf{54.8}&\textbf{42.1} &\textbf{65.6}& \textbf{75.1}& 68.6& \textbf{65.5}\\ 
\multicolumn{1}{c|}{} &\textbf{(1.6)}&\textbf{(1.5)}&\textbf{(2.5)}&\textbf{(2.3)}&\textbf{(1.4)}&\textbf{(0.5)}&\textbf{(1.4)}&(0.7)&\textbf{(0.8)}&\textbf{(1.3)}&\textbf{(1.1)}&\textbf{(1.4)}&(2.9)&\textbf{(1.0)}\\\bottomrule
\end{tabular}%
}
\caption{We report results on three different real-world datasets with format mean(std) from 5-trial run. For Office-Caltech 10, \textit{A, C, D ,W} are abbreviations for Amazon, Caltech, DSLR and WebCam, for DomainNet, \textit{C, I, P, Q, R, S} are abbreviations for Clipart, Infograph, Painting, Quickdraw, Real and Sketch. For ABIDE, we list the abbreviations for the clients (i.e., medical institutions).
%\Xiaoxiao{Change the order of abide and domainnet, bolden the best result}
}
\label{tab:my-table}
\vspace{-3mm}
\end{table}


\paragraph{Datasets and Setup:} (1) We conduct the classification task on natural images from \textit{Office-Caltech10}, which has four data sources composing Office-31 \cite{saenko2010adapting} (three data sources) and Caltech-256 datasets (one data source) \cite{griffin2007caltech}, which are acquired using different camera devices or in different real environment with various background. \revision{Each client joining the FL system is assigned data from one of the four data sources. Thus data is non-iid across the clients.} 
(2) Our second dataset is \textit{DomainNet}, which contains natural images coming from six different data sources: Clipart, Infograph, Painting, Quickdraw, Real, and Sketch. \revision{Similar to (1), each client contains iid data from one of the data sources, but clients with different data sources have different feature distributions.} (3) We include four medical institutions (NYU, USM, UM, UCLA; each is viewed as a client) from \textit{ABIDE I} that collects functional brain images using different imaging equipment and protocols. We validate on a medical application for binary classification between autism spectrum disorders patients and healthy control subjects. 
 
The Office-Caltech10 contains ten categories of objects. The DomainNet extensively contains 345 object categories and we use the top ten most common classes to form a sub-dataset for our experiments.
%and DomainNet, we use the top 10 common objects among their sub-datasets. 
Our classification models adopt AlexNet \citep{krizhevsky2012imagenet} architecture with BN added after each convolution and fully-connected layer. Before feeding into the network, all images are resized to $256\times256\times3$. For ABIDE I, each instance is represented as a 5995-dimensional vector through brain connectome computation. 
%The task we performed on ABIDE is a binary classification for ASD v.s. HC. 
We use a three-layer fully connected neural network as the classifier with the hidden layers of 16 with two BN layers after the first two fully connected layers. Same as the above benchmark, we perform 5 repeated runs for each experiment. 
 
 
\textbf{Results and Analysis:}
The experimental results are shown in Table \ref{tab:my-table} in the form of mean (std). On Office-Caltech10, FedBN significantly outperforms the state-of-the-art method of FedProx, and improves at least $6\%$ on mean accuracy compared with all the alternative methods. On DomainNet, FedBN achieved supreme accuracy over most of the datasets. Interestingly, we find the alternative FL methods achieves comparable results with SingleSet except Quickdraw, and FedBN outperforms them over $10\%$.  
Surprisingly, for the above two tasks, the alternative FL strategies are ineffective in the feature shift non-iid datasets, even worse than using single client data for training for most of the clients. In ABIDE I, FedBN excell by a non-negligible margin on three clients regarding the mean testing accuracy. The results are inspiring and bring the hope of deploying FedBN to healthcare field, where data are often limited, isolated and heterogeneous on features.






==> Federated Learning for Non-IID Data/future.tex <==
\section{Discussion and Future Work}

\Xiaoxiao{This is a first draft for the discussion. It is far from good. Your comments are very welcome!}

In classical federated learning, a new client can be added to a system by initializing this client with the current global parameters. In FedBN, however, the BN parameters are not shared. This issue can be overcome by sharing BN parameters as well and initializing a new client with the average BN parameters. We detail this approach in Appendix~\ref{app:test}.

FedBN is independent of the optimization strategy, communication scheme, and the aggregation technique. Thus, it can be used with various optimizers~\citep{}, efficient communication schemes (e.g., averaging random subsets~\citep{mcmahan2017communication}, dynamic averaging~\citep{kamp2019black}),%, or compression~\citep{suresh2017distributed}),
and aggregation techniques (e.g., geometric median~\citep{pillutla2019robust}, Radon machines~\citep{kamp2017effective}, or distributed distillation~\citep{bistritz2020distributed}).

Since batch normalization is often applied in multiple layers within a network architecture, normalization affects different representations of the data and thus allows for a more complex normalization than usual forms of data preprocessing. Thus, we believe that FedBN improves a wide range of applications, most prominently autonomous driving and healthcare. In both cases, local clients might capture data using different sensors or equipment (sensor types vary between vehicle types or generations, in hospitals the imaging equipment can vary). An interesting direction for future work is analyzing what types of differences in local data can be ironed out by FedBN and where the limits of the method lie. Moreover, not sharing local BN parameters should make inference on local data more challenging. It would be interesting to quantify this improvement in privacy.

\begin{enumerate}
    \item Privacy
    \item Healthcare
    \item Methods (whether BN can be replaced with other normalization)
    \item Aggregate BN using clustering. 
    \item Contact MONAI and Clara
    \item Camera Ready -- 1. Future work: the methods can be intergrated with other optimization strategy such as FedAdam, aggregating strategies.  2. Put a table with combination results. 3. Proof-reading the manuscript. 
    \item Add out of domain client case in discussion session but do not include the table.
    \item Add ``sharing BN parameters will cause higher communication costs and privacy issues'' to some where.
\end{enumerate}

==> Federated Learning for Non-IID Data/illustration.tex <==






==> Federated Learning for Non-IID Data/introdcution.tex <==
\section{Introduction}


Federated learning (FL), has gained popularity for various applications involving learning from distributed data.
In FL, a cloud server (the “server”) can communicate with distributed data sources (the “clients”), while the clients hold data separately.  A major challenge in FL is the training data statistical heterogeneity among the clients \citep{kairouz2019advances, li2018federated}. 
It has been shown that standard federated methods such as FedAvg \citep{mcmahan2017communication} which are not designed particularly taking care of non-iid data significantly suffer from performance degradation or even diverge if deployed over non-iid samples \citep{karimireddy2019scaffold,li2018adaptive,li2020federated}.



Recent studies have attempted to address the problem of FL on non-iid data. Most variants of FedAvg primarily tackle the issues of stability, client drift and heterogeneous label distribution over clients \citep{li2018federated, karimireddy2019scaffold, zhao2018federated}. Instead, we focus on the shift in the feature space, which has not yet been explored in the literature. Specifically, we consider that local data deviates in terms of the distribution in feature space, and identify this scenario as \textit{feature shift}. 
This type of non-iid data is a critical problem in many real-world scenarios, typically in cases where the local devices are responisble for a heterogeneity in the feature distributions. For example in cancer diagnosis tasks, medical radiology images collected in different hospitals have uniformly distributed labels (i.e., the cancer types treated are quite similar across the hospitals). However, the image appearance can vary a lot due to different imaging machines and protocols used in hospitals, e.g., different intensity and contrast.
In this example, each hospital is a client and hospitals aim to collaboratively train a cancer detection model without sharing privacy-sensitive data.


Tackling non-iid data with feature shift has been explored in classical centralized training in the context of domain adaptation. Here, an effective approach in practice is utilizing Batch Normalization (BN)~\citep{ioffe2015batch}: recent work has proposed BN as a tool to mitigate domain shifts in domain adaptation tasks  with promising results achieved~\citep{li2016revisiting,liu2020ms, chang2019domain}. Inspired by this, this paper proposes to apply BN for feature shift FL. To illustrate the idea, we present a toy example that illustrates how BN may help harmonizing local feature distributions.


\paragraph{Observation of BN in a FL Toy Example:} 
We consider a simple non-convex learning problem: we generate data $x,y\in\mathbb{R}$ with $y=\cos(w_{true}x)+\epsilon$, where $x\in\mathbb{R}$ is drawn iid from Gaussian distribution and $\epsilon$ is zero-mean Gaussian noise and consider models of the form $f_w(x) = \cos(wx)$ with model parameter $w\in\mathbb{R}$. 
Local data deviates in the variance of $x$.
First, we illustrate that local batch normalization harmonizes local data distributions. 
We consider a simplified form of BN that normalizes the input by scaling it with $\gamma$, i.e., the local empirical standard deviation, and a setting with 2 clients.
As Fig.~\ref{fig:illustration:trainLossCl1Cl2} shows, the local squared loss is very different between the two clients. Thus, averaging the model does not lead to a good model.
However when applying local BN, the local training error surfaces become similar and averaging the models can be beneficial. To further illustrate the impact of BN, we plot the error surface  for one client with respect to both model parameter $w\in\mathbb{R}$ and BN parameter $\gamma\in\mathbb{R}$ in Fig.~\ref{fig:illustration:3DplotCl1}. The figure shows that for an optimal weight $w_1^*$, changing $\gamma$ deteriorates the model quality. Similarly, for a given optimal BN parameter $\gamma_1^*$, changing $w$ deteriorates the quality. In particular, the average model $\overline{w}=(w_1^*+w_2^*)/2$ and average BN parameters $\overline{\gamma}=(\gamma_1^*+\gamma_2^*)/2$ has a high \revision{generalization} error. At the same time, the average model $\overline{w}$ with local BN parameter $\gamma_1^*$ performs very well.


\begin{figure}[t]
	\begin{minipage}[t]{.48\textwidth}
		\centering
		\includegraphics[width=\textwidth]{trainLossWithAndWithoutBN.pdf}
		\vspace{-4mm}
		\captionof{figure}{Training error on local datasets for two clients respectively with and w/o BN, where BN harmonizes the loss surface.}
		\label{fig:illustration:trainLossCl1Cl2}
	\end{minipage}
	\hfill
	\begin{minipage}[t]{.48\textwidth}
		\centering
		\includegraphics[width=\textwidth]{3dplot_Client1.pdf}
		\vspace{-4mm}
		\captionof{figure}{Error surface of a client for model parameter $w\in[0.001,12]$ and BN parameter $\gamma\in [0.001,4]$. Averaging model \emph{and} BN parameters leads to worse solutions.}
		\label{fig:illustration:3DplotCl1}
	\end{minipage}  
	\label{fig:illustration}
	
	\vspace{-5mm}
\end{figure}

Motivated by the above insight and observation, this paper proposes a novel federated learning method, called FedBN, for addressing non-iid training data which keeps the client BN layers updated locally, without communicating, and aggregating them at the server. In practice, we can simply update the non-BN layers using FedAvg, without modifying any optimization or aggregation scheme. This approach has zero parameters to tune, requires minimal additional computational resources, and can be easily applied to arbitrary neural network architectures with BN layers in FL. Besides the benefit shown in the toy example, we also show the benefits in accelerating convergence by theoretically analyzing the convergence of FedBN in the over-parameterized regime. In addition, we have conducted extensive experiments on a benchmark and three real-world datasets. 
Compared to classical FedAvg, as well as the state-of-the-art for non-iid data (FedProx), our novel method, FedBN, demonstrates significant  practical improvements on the extensive experiments. 








==> Federated Learning for Non-IID Data/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Federated Learning for Non-IID Data/method.tex <==
\section{Federated Averaging with Local Batch Normalization}
\label{sec:method}

\subsection{Proposed Method - FedBN}
We propose an efficient and effective learning strategy denoted \textit{FedBN}. Similar to FedAvg, FedBN performs local updates and averages local models. However, FedBN assumes local models have BN layers and excludes their parameters from the averaging step. We present the full algorithm in Appendix~\ref{sec:appalgorithm}.
This simple modification results in significant empirical improvements in non-iid settings. We provide an explanation for these improvements in a simplified scenario, in which we show  that FedBN improves the convergence rate under feature shift. 

\iffalse
\paragraph{Notation} 
Let $\b x^i$ denote the training point from client $i \in [N]$, i.e. $\b x^i = \b x \cdot \bm{1}\{\b x \in \text{client } i\}$. 
Let $\b v_k \in \R^d$, $k = 1, \dots, m$ denote the parameters of the first layer, and let $m$ denote the width of the hidden layer.
Let $\parallel \b v \parallel_2$ denote the $l_2$ norm for a vector $\b v$, and let $\parallel \b v \parallel_S \triangleq \sqrt{\b v^\top S \b v}$ denote the induced vector norm for a positive definite matrix $S$.
Let ReLU activation function be $\sigma (s) = \max\{s,0\}$. 
\fi


\subsection{Problem Setup}
We assume $N\in\mathbb{N}$ clients to jointly train for $T\in\mathbb{N}$ epochs and to communicate after $E\in\mathbb{N}$ local iterations. Thus, the system has $\sfrac{T}{E}$ communication rounds over the $T$ epochs. For simplicity, we assume all clients to have $M\in\mathbb{N}$ training examples (a difference in training examples can be account for by weighted averaging~\citep{mcmahan2017communication}) for a regression task, i.e., each client $i \in [N]$ ($[N] = \{1,\dots,N\}$) has training examples $\{(\b x^i_j, y^i_j)\in \R^d \times \R: j \in [M]\}$. Furthermore, we assume a two-layer neural network with ReLU activations trained by gradient descent. Let $\b v_k \in \R^d$ denote the parameters of the first layer, where $k \in [m]$ and $m$ is the width of the hidden layer.
Let $\parallel \b v \parallel_{\b S} \triangleq \sqrt{\b v^\top \b S \b v}$ denote the induced vector norm for a positive definite matrix $\b S$. 


\revision{We consider a non-iid setting in FL where local feature distributions differ---not label distribution, as considered, e.g., in~\cite{mcmahan2017communication,li2019convergence}.}
To be more precise, we make the following assumption. 
\begin{assumption}[Data Distribution]
\label{as:data}
For each client $i \in [N]$ the inputs $\b x^i_j$ are centered $(\E \b x^i = \b 0)$ with covariance matrix $\b S_i = \E \b x^i \b x^{i\top} $, where $\b S_i$ is independent from the label $\b y$ and may differ for each $i\in [N]$ e.g., $\b S_i$ are not all identity matrices, and for each index pair $p \neq q$, $\b x_p \neq \kappa \cdot \b x_q$ for all $\kappa \in \R \setminus \{0\}$.
\end{assumption}

With Assumption \ref{as:data}, the normalization of the first layer for client $i$ is $ \frac{\b v_k^\top \b x^i}{\parallel \b v_k \parallel_{\b S_i}}$. FedBN with client-specified BN parameters trains a model $f^*: \R^d \rightarrow \R$ parameterized by $(\b V, \mathbf{\gamma}, \b c) \in \R^{m \times d} \times \R^{m \times N} \times \R ^m$, i.e., 
\begin{align}
\label{equ: fedbn}
f^*(\b x; \b V, \mathbf{\gamma}, \b c) = 
\frac{1}{\sqrt{m}} \sum^m_{k=1}c_k \sum_{i=1}^N \sigma\left(\gamma_{k,i} \cdot \frac{\b v_k^\top \b x}{\parallel \b v_k \parallel_{\b S_i}}\right) \cdot \bm{1}\{\b x \in \text{client } i\} \enspace,
\end{align}
where $\mathbf{\gamma}$ is the scaling parameter of BN and $\sigma (s) = \max\{s,0\}$ is the ReLU activation function, $\b c$ is the top layer parameters of the network. Here, we omit learning the shift parameter of BN \footnote{
We omit centering neurons as well as learning the shift parameter of BN for the neural network analysis because of the assumption that $\b x$ is zero-mean and the two layer network setting \citep{kohler2019exponential,salimans2016weight}.}. FedAvg instead trains a function $f: \R^d \rightarrow \R$ which is a special case of Eq.~\ref{equ: fedbn} with $\gamma_{k,i} = \gamma_{k}$ for $\forall i \in [N]$.
%
We take a random initialization of the parameters \citep{salimans2016weight} in our analysis:
\begin{align}
\label{equ: inti}
\mathbf{v}_{k}(0) \sim N\left(0, \alpha^{2} \mathbf{I}\right), \quad c_{k} \sim U\{-1,1\}, 
\quad \text{and} \quad \gamma_{k} = \gamma_{k,i} = \left\|\mathbf{v}_{k}(0)\right\|_{2} / \alpha,
\end{align}
where
$\alpha^2$ controls the magnitude of $\b v_k$ at initialization. The initialization of the BN parameters $\gamma_k$ and $\gamma_{k,i}$ are independent of $\alpha$. The parameters of the network $f^*(\b x; \b V, \mathbf{\gamma}, \b c)$ are obtained by minimizing the empirical risk with respect to the squared loss using gradient descent :
\begin{align}
    % \min_{\b w \in \mathcal{W}} 
   L(f^*) = \frac{1}{NM}\sum_{i=1}^N\sum_{j=1}^M \left(f^*(\b x_j^i)-y_j^i\right)^2 \enspace .
   \label{eq:loss} 
\end{align}  


\iffalse 
With the Assumption \ref{as:data}, the normalization of the first layer for client $i$ is
\begin{align*}
      \frac{\b v_k^\top \b x^i - -E(\b v_k^\top \b x^i)}{\sqrt{\E (\b v_k^\top \b x^i \b x^{i\top} \b v_k)}} 
     =   \frac{\b v_k^\top \b x^i}{\sqrt{ \b v_k^\top \b S_i \b v_k}}
     =   \frac{\b v_k^\top \b x^i}{\parallel \b v_k \parallel_{\b S_i}}.
\end{align*}

Then, FedAvg trains a function $f: \R^d \rightarrow \R$ parameterized by $(\b V, \mathbf{\gamma}, \b c) \in \R^{m \times d} \times \R^{m} \times \R ^m$ that 
\begin{align}
\label{equ: fedavg}
f(\b x; \b V, \mathbf{\gamma}, \b c) = 
\frac{1}{\sqrt{m}} \sum^m_{k=1}c_k \sum_{i=1}^N \sigma(\gamma_k \cdot \frac{\b v_k^\top \b x^i}{\parallel \b v_k \parallel_{\b S_i}}),
\end{align}
where the output is normalized by factor $\sqrt{m}$. And FedBN with locally specified BN layers, trains a function $f^*: \R^d \rightarrow \R$ parameterized by $(\b V, \mathbf{\gamma}, \b c) \in \R^{m \times d} \times \R^{m \times N} \times \R ^m$ that 
\begin{align}
\label{equ: fedbn}
f^*(\b x; \b V, \mathbf{\gamma}, \b c) = 
\frac{1}{\sqrt{m}} \sum^m_{k=1}c_k \sum_{i=1}^N \sigma(\gamma_{k,i} \cdot \frac{\b v_k^\top \b x^i}{\parallel \b v_k \parallel_{\b S_i}}).
\end{align}
In each batch, BN decomposes the weight vector into magnitude and direction.

In the training, we take a random initialization of the parameters \citep{salimans2016weight}:
\begin{align}
\label{equ: inti}
\mathbf{v}_{k}(0) \sim N\left(0, \alpha^{2} \mathbf{I}\right), \quad c_{k} \sim U\{-1,1\}, 
\quad \text{and} \quad \gamma_{k} = \gamma_{k,i} = \left\|\mathbf{v}_{k}(0)\right\|_{2} / \alpha,
\end{align}
where $\alpha^2$ controls the magnitude of $\b v_k$ at initialization. The initialization of the magnitude parameters $\gamma_k$ and $\gamma_{k,i}$ are independent of $\alpha$. The parameters in networks (\ref{equ: fedavg}) and (\ref{equ: fedbn}) are optimized using the $NM$ training samples respectively on the square loss function.
\fi
\vspace{-2mm}
% \textbf{Convergence Analysis:} 
\subsection{Convergence Analysis} 
Here we study the trajectory of networks FedAvg ($f$) and FedBN ($f^*$)'s prediction through the neural tangent kernel (NTK) introduced by \cite{jacot2018neural}. Recent machine learning theory studies \citep{arora2019fine,du2018gradient,allen2019convergence,van2020training,dukler2020optimization} have shown that for finite-width over-parameterized networks, the convergence rate is controlled by the least eigenvalue of the induced kernel in the training evolution. 

To simplify tracing the optimization dynamics, we consider the case that the number of local updates $E$ is $1$. 
We can decompose the NTK into a magnitude component $\mathbf{G}(t)$ and direction component $\mathbf{V}(t) / \alpha^{2}$ following \cite{dukler2020optimization}:
\begin{align*}
\frac{d \mathbf{f}}{d t}=-\mathbf{\Lambda}(t)(\mathbf{f}(t)- \b y), \quad \text{where} \quad
\mathbf{\Lambda}(t):=\frac{\mathbf{V}(t)}{\alpha^{2}}+\mathbf{G}(t).
\end{align*}
The specific forms of $\mathbf{V}(t)$ and $\mathbf{G}(t)$ are given in Appendix \ref{sec:evol}. 
Let $\lambda_{min} (A)$ denote the minimal eigenvalue of matrix $A$. The matrices $\mathbf{V}(t)$ and $\mathbf{G}(t)$ are positive semi-definite, since they can be viewed as covariance matrices. This gives $
\lambda_{\min }(\mathbf{\Lambda}(t)) \geq \max \left\{\lambda_{\min }(\mathbf{V}(t)) / \alpha^{2}, \lambda_{\min }(\mathbf{G}(t))\right\}$.
According to NTK, the convergence rate is controlled by $\lambda_{min} (\mathbf{\Lambda}(t))$. 
Then, for $\alpha > 1$, convergence is dominated by $\b G(t)$. Let $\mathbf{\Lambda}(t)$ and $\mathbf{\Lambda}^*(t)$ denote the evolution dynamics of FedAvg and FedBN and let $\mathbf{G}(t)$ and $\mathbf{G}^*(t)$ denote the magnitude component in the evolution dynamics of FedAvg and FedBN.
%
For the convergence analysis, we use the auxiliary version of the Gram matrices, which is defined as follows. 
\begin{definition}
Given sample points $\{\b x_p\}_{p=1}^{NM}$, we define the auxiliary Gram matrices $\mathbf{G}^{\infty}  \in \R^{NM \times NM}$ and $\mathbf{G}^{*\infty}  \in \R^{NM \times NM}$ as
\begin{align}
\mathbf{G}_{p q}^{\infty} & := \mathbb{E}_{\mathbf{v} \sim N\left(0, \alpha^{2} \mathbf{I}\right)}
 \sigma\left(\mathbf{v}^{\top} \mathbf{x}_{p}\right) \sigma\left(\mathbf{v}^{\top} \mathbf{x}_{q}\right), \label{equ: fedavg_g} ~~~\text{(FedAvg)}  \\
 \mathbf{G}_{p q}^{*\infty} & := \mathbb{E}_{\mathbf{v} \sim N\left(0, \alpha^{2} \mathbf{I}\right)}
 \sigma\left(\mathbf{v}^{\top} \mathbf{x}_{p}\right) \sigma\left(\mathbf{v}^{\top} \mathbf{x}_{q}\right) \bm{1}\{i_p = i_q\}, ~~~\text{(FedBN)} \label{equ: fedbn_g} . 
\end{align}
\end{definition}
Given Assumption~\ref{as:data}, we use the key results in \cite{dukler2020optimization} to show that $\b G^{\infty}$ is positive definite. Further, we show that $\b G^{*\infty}$ is positive definite. We use the fact that the distance between $\b G(t)$ and its auxiliary version is small in over-parameterized neural network, such that $\b G(t)$ remains positive definite.

\begin{lemma} 
\label{lemma:eigen}
Fix points $\{\b x_p\}_{p=1}^{NM}$ satisfying Assumption~\ref{as:data}. Then Gram matrices $\mathbf{G}^{\infty} $ and $\mathbf{G}^{*\infty} $ defined as in (\ref{equ: fedavg_g}) and (\ref{equ: fedbn_g}) are strictly positive definite. Let the least eigenvalues be $\lambda_{\min}(\b G^{\infty}) =: \mu_0$ and $\lambda_{\min}(\b G^{*\infty}) =: \mu^*_0,$ where $\mu_0,\mu_0^*>0$.
\end{lemma}
\vspace{-2mm}
\paragraph{Proof sketch} The main idea follows \cite{du2018gradient,dukler2020optimization}, that given points $\{\b x_p\}_{p=1}^{NM}$, the matrices $\mathbf{G}^{\infty} $ and $\mathbf{G}^{*\infty}$ can be shown as covariance matrix of linearly independent operators. More details of the proof are given in the Appendix \ref{sec:proof_lemma}.

\revision{Based on our formulation, the convergence rate of FedAvg (Theorem \ref{th:converge_g}) can be derived from \cite{dukler2020optimization} by considering non-identical covariance matrices.} We derive the convergence rate of FedBN in Corollary \ref{th:converge_fedbn}. Our key result of comparing the convergence rates between FedAvg and FedBN is culminated in Corollary \ref{coro:comp}.
\vspace{-1mm}
\begin{theorem}[$\b G$-dominated convergence for FedAvg \cite{dukler2020optimization}]
\label{th:converge_g}
Suppose network (\ref{equ: fedavg_g}) is initialized as in (\ref{equ: inti}) with $\alpha >1$, trained using gradient descent and Assumptions \ref{as:data} holds. Given the loss function of training the neural network is the square loss with targets $\b y$ satisfying $\|\mathbf{y}\|_{\infty}=O(1)$. If $m=\Omega\left(\max \left\{N^{4}M^{4} \log (NM / \delta) / \alpha^{4} \mu_{0}^{4}, N^{2}M^2 \log (NM / \delta) / \mu_{0}^{2}\right\}\right)$, then with probability $1-\delta$,
\begin{enumerate}
\item For iterations $t = 0, 1, \cdots$, the evolution matrix $\mathbf{\Lambda}(t)$ satisfies $\lambda_{\min }(\mathbf{\Lambda}(t)) \geq \frac{\mu_{0}}{2}$.
% , and $\mathbf{\Lambda}^*(t)$ satisfies $\lambda_{\min }(\mathbf{\Lambda}^*(t)) \geq \frac{\mu^*_{0}}{2}$.
\item Training with gradient descent of step-size $\eta = O\left(\frac{1}{\|\mathbf{\Lambda}(t)\|}\right)$ converges linearly as
\begin{align*}
\|\mathbf{f}(t)-\mathbf{y}\|_{2}^{2} \leq \left(1-\frac{\eta \mu_{0}}{2}\right)^{t}\|\mathbf{f}(0)-\mathbf{y}\|_{2}^{2}. 
\end{align*}

\end{enumerate}
\end{theorem}
Following the key ideas in \cite{dukler2020optimization}, here we further characterize the convergence for FedBN.  
\begin{corollary}[$\b G$-dominated convergence for FedBN]
\label{th:converge_fedbn}
Suppose network (\ref{equ: fedbn_g}) and all other conditions in Theorem \ref{th:converge_g}. With probability $1-\delta$, for iterations $t = 0, 1, \cdots$, the evolution matrix $\mathbf{\Lambda}^*(t)$ satisfies $\lambda_{\min }(\mathbf{\Lambda}^*(t)) \geq \frac{\mu^*_{0}}{2}$ and training with gradient descent of step-size $\eta = O\left(\frac{1}{\|\mathbf{\Lambda}^{*}(t)\|}\right)$ converges linearly as $\|\mathbf{f}^*(t)-\mathbf{y}\|_{2}^{2} \leq \left(1-\frac{\eta \mu^*_{0}}{2}\right)^{t}\|\mathbf{f}^*(0)-\mathbf{y}\|_{2}^{2}$.
\end{corollary}
The exponential factor of convergence for FedAvg $\left(1-\eta \mu_{0}/2\right)$ and FedBN $\left(1-\eta \mu^*_{0}/2\right)$ are controlled by the smallest eigenvalue of $
\b G(t)$, respectively $\b G^*(t)$. Then we can analyze the convergence performance of FedAvg and FedBN by comparing $\lambda_{\min}(\b G^{\infty})$ and $\lambda_{\min}(\b G^{*\infty})$. 

\begin{corollary}[Convergence rate comparison between FedAvg and FedBN]
\label{co:46}
For the $\b G$-dominated convergence, the convergence rate of FedBN is faster than that of FedAvg. 
\label{coro:comp}
\end{corollary} 
\vspace{-3mm}
\paragraph{Proof sketch} The key is to show $\lambda_{\min}(\b G^{\infty}) \leq \lambda_{\min}(\b G^{*\infty})$. Comparing equation (\ref{equ: fedavg_g}) and (\ref{equ: fedbn_g}), $\b G^{*\infty}$ takes the $M \times M$ block matrices on the diagonal of $\b G^{\infty}$. Let $\b G^{\infty}_i$ be the $i$-th $M \times M$ block matrices on the diagonal of $\b G^{\infty}$. By linear algebra, $\lambda_{\min}(\b G^{\infty}_i) \geq \lambda_{\min}(\b G^{\infty})$ for $i \in [N]$. Since $\b G^{*\infty} = diag(\b G^{\infty}_1,\cdots,\b G^{\infty}_N)$, we have $\lambda_{\min}(\b G^{*\infty}) = \min_{i \in [N]} \{ \lambda_{\min}(\b G^{\infty}_i) \}$. Therefore, we have the result $\lambda_{\min}(\b G^{*\infty}) \geq \lambda_{\min}(\b G^{\infty})$.



==> Federated Learning for Non-IID Data/notations.tex <==
\section*{Appendix}
\paragraph{Roadmap of Appendix} The Appendix is organized as follows.
We list the notations table in Section~\ref{app:notation}.
We provide theoretical proof of convergence in Section~\ref{app:proof}. 
The algorithm of FedBN is described in Section~\ref{app:algorithm}.
The details of experimental setting are in Section~\ref{app:detail} and additional results on benchmark datasets are in Section~\ref{sec:morebench}. We show experiment on synthetic data in Section~\ref{app:synth}. We demonstrate the ability of generalizing FedBN to test on a new client in Section~\ref{app:test}.

\section{Notation Table}
\label{app:notation}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cl}
\hline
Notations & Description \\ \hline
$\b x$ & features, $\b x \in \R^d$ \\
$d$ & dimension of $\b x$ \\
$y$ & labels, $y \in \R$  \\
$P(\cdot)$ & probability distribution \\
$N$ & total number of clients \\
$T$ & total number of epochs in training \\
$E$ & number of local iteration in FL \\
$M$ & number of training samples in each client \\
$[N]$ & set of numbers, $[N] = \{1,\dots,N\}$ \\
$i$ & indicator for client, $i \in [N]$ \\
$j$ & indicator for sample in each client, $j \in [M]$ \\
$(\b x^i_j, y^i_j)$ & the $j$-th training sample in client $i$ \\
$m$ & number of neurons in the first layer \\
$k$ & indicator for neuron, $k \in [m]$ \\
$\b v_k$ & parameters for the $k$-th neuron in the first layer \\
$\parallel \b v \parallel_{\b S} $ & vector norm, $\parallel \b v \parallel_{\b S} \triangleq \sqrt{\b v^\top \b S \b v}$, given a matrix $\b S$ \\
$\b S_i$ & covariance matrix for features in client $i$, $\b S_i = \E \b x^i \b x^{i\top} $ \\
$p,q$ & indicator for sample, $p,q \in [NM]$ \\
$f$ & two layer ReLU neural network with BN \\
$f^*$ & two layer ReLU neural network with BN with client-specified BN parameters \\
$\b V$ & parameters of the first phase neurons, $\b V \in \R^{m \times d}$  \\ 
$\boldsymbol{\gamma}$ & the scaling parameter of BN \\
$\b c$ & top layer parameters of the network \\
$\sigma(\cdot)$ & ReLU activation function, $\sigma(\cdot) = \max\{\cdot,0\}$ \\
$N (\boldsymbol{\mu}, \boldsymbol{\Sigma})$ & Gaussian with mean $\boldsymbol{\mu}$ and covariance $\boldsymbol{\Sigma}$ \\
$U[-1,1]$ & Rademacher distribution \\
$\alpha$ & variance of $\b v_k$ at initialization \\
$L(f)$ & empirical risk with square loss for network $f$ \\
$\boldsymbol{\Lambda}(t)$ & evolution dynamic for FedAvg at epoch $t$ \\
$\b V(t)$ & evolution dynamic with respect to $\b V$ for FedAvg at epoch $t$ \\
$\b G(t)$ & evolution dynamic with respect to $\boldsymbol{\gamma}$ for FedAvg at epoch $t$ \\
$\boldsymbol{\Lambda}^*(t)$ & evolution dynamic for FedBN at epoch $t$ \\
$\b V^*(t)$ & evolution dynamic with respect to $\b V$ for FedBN at epoch $t$ \\
$\b G^*(t)$ & evolution dynamic with respect to $\boldsymbol{\gamma}$ for FedBN at epoch $t$ \\
$\lambda_{min}(A)$ & the minimal eigenvalue of matrix $A$ \\
$\b G^{\infty}$ & expectation of $\b G(t)$ \\
$\b G^{*\infty}$ & expectation of $\b G^*(t)$ \\
\hline
\end{tabular}%
}
\caption{Notations occurred in the paper.}
\label{tab:notation}
\end{table}

==> Federated Learning for Non-IID Data/preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}

\textbf{Non-IID Data in Federated Learning:} We introduce the concept of \textit{feature shift} in federated learning as a novel category of client's non-iid data distribution. So far, the categories of non-iid data considered according to \cite{kairouz2019advances, hsieh2019non} can be described by the joint probability between features $\b x$ and labels $y$ on each client. We can rewrite $P_i(\b x,y)$  as  $P_i(y|\b x)P_i(\b x)$ and $P_i(\b x|y)P_i(y)$. We define \textit{feature shift} as the case that covers: 1)~\textit{covariate shift}:  the marginal distributions $P_i(\b x)$ varies across clients, even if $P_i(y|\b x)$ is the same for all client; and 2)~\textit{concept shift}: the conditional distribution $P_i(\b x|y)$ varies across clients and $P(y)$ is the same. 
\textbf{Federated Averaging (FedAvg):} 
We establish our algorithm on FedAvg introduced by \cite{mcmahan2017communication} which is the most popular existing and easiest to implement federated learning strategy, where clients collaboratively send updates of locally trained models to a global server. Each client runs a local copy of the global model on its local data. The global model's weights are then updated with an average of local clients' updates and deployed back to the clients. This builds upon previous distributed learning work by not only supplying local models but also performing training locally on each device. Hence FedAvg potentially empowers clients (especially clients with small dataset) to collaboratively learn a shared prediction model while keeping all training data locally. Although FedAvg has shown successes in classical Federated Learning tasks, it suffers from slow convergence and low accuracy in most non-iid contents \citep{li2018federated,li2019convergence}. 






==> Federated Learning for Non-IID Data/related.tex <==
\section{Related Work}
\label{sec:related_work}

\paragraph{Techniques for Non-IID Challenges in Federated Learning:}
The widely known aggregation strategy in FL, FedAvg \citep{mcmahan2017communication}, often suffers when data is heterogeneous over local client. 
Empirical work addressing non-iid issues, mainly focus on label distribution skew, where a non-iid dataset is formed by partitioning a “flat” existing dataset based on the labels. 
FedProx \citep{li2018federated}, a recent framework tackled the heterogeneity by allowing partial information aggregation and adding a proximal term to FedAvg. \cite{zhao2018federated}
assumed a subset of the data is globally shared between all the clients, hence generalizes to the problem at hand. FedMA \citep{wang2020federated} proposed an aggregation strategy for non-iid data partition that shares global model in a layer-wise manner. However, so far there are only limited attempts considering non-iid induced from feature shift, which is common in medical data collecting from different equipment and natural image collected in various noisy environment. Very recently, FedRobust \citep{reisizadeh2020robust} assumes data follows an affine distribution shift and tackles this problem by learning the affine transformation. This hampers the generalization when we cannot estimate the explicit affine transformation. \revision{Concurrently to our work, SiloBN \cite{andreux2020siloed} empirically shows that local clients keeping some untrainable BN parameters could improve robustness to data heterogeneity, but provides no theoretical analysis of the approach. FedBN instead keeps all BN parameters strictly local. Recently, an orthogonal approach to the non-iid problem has been proposed that focuses on improving the optimization mechanism~\citep{reddi2020adaptive,zhang2020fedpd}.}

\paragraph{Batch Normalization in Deep Neural Networks:} 
Batch Normalization~\citep{ioffe2015batch} is an indispensable component in many deep neural networks and has shown its success in neural network training. Relevant literature has uncovered a number of benefits given by batch normalization. \cite{santurkar2018does} showed that BN makes the optimization landscape significantly smoother. \cite{luo2018towards} investigated an explicit regularization form of BN such that improving the robustness of optimization. \cite{morcos2018importance} suggested that BN implicitly discourages single direction
reliance, thus improving model generalizability. \cite{li2018adaptive} took advantage of BN for tackling the domain adaptation problem. However, what a role BN is playing in the scope of federated learning, especially for non-iid training, still remains unexplored to date. 




==> Federated Learning for Non-IID Data/theory.tex <==
\newpage
\section{Convergence Proof}
\label{app:proof}
\subsection{Evolution Dynamics}
\label{sec:evol}
In this section, we calculate the evolution dynamics $\boldsymbol{\Lambda}(t)$ for training with function $f$ and $\boldsymbol{\Lambda}^*(t)$ for training with $f^*$. 
Since the parameters are updated using gradient descent, the optimization dynamics of parameters are
\begin{align*}
\frac{d \mathbf{v}_{k}}{d t}=-\frac{\partial L}{\partial \mathbf{v}_{k}}, \quad \frac{d \gamma_{k}}{d t}=-\frac{\partial L}{\partial \gamma_{k}}.
\end{align*}
Let $f_p = f(\b x_p^{i_p})$. Then, the dynamics of the prediction of the $p$-th data point in site $i_p$ is 
\begin{align*}
\frac{\partial f_{p}}{\partial t}
=\sum_{k=1}^{m} \frac{\partial f_{p}}{\partial \mathbf{v}_{k}} \frac{d \mathbf{v}_{k}}{d t}+\frac{\partial f_{p}}{\partial \gamma_{k}} \frac{d \gamma_{k}}{d t}
=-\underbrace{\sum_{k=1}^{m} \frac{\partial f_{p}}{\partial \mathbf{v}_{k}} \frac{\partial L}{\partial \mathbf{v}_{k}}}_{T_{\mathbf{v}}^{p}}-\underbrace{\sum_{k=1}^{m} \frac{\partial f_{p}}{\partial \gamma_{k}} \frac{\partial L}{\partial \gamma_{k}}}_{T_{\gamma}^{p}}.
\end{align*}
The gradients of $f_p$ and $L$ with respect to $\b v_k$ and $\gamma_k$ are computed as
\begin{align*}
\begin{aligned}
\frac{\partial f_{p}}{\partial \mathbf{v}_{k}}(t) &=\frac{1}{\sqrt{m}} \frac{c_{k} \cdot \gamma_{k}(t)}{\left\|\mathbf{v}_{k}(t)\right\|_{\b S_{i_p}}} \cdot \b x_{p}^{\mathbf{v}^{i_p}_{k}(t)^{\perp}} \bm{1}_{p k}(t), \\
\frac{\partial L}{\partial \mathbf{v}_{k}}(t) &=\frac{1}{\sqrt{m}} \sum_{q=1}^{N M}\left(f_{q}(t)-y_{q}\right) \frac{c_{k} \cdot \gamma_{k}(t)}{\left\|\mathbf{v}_{k}(t)\right\|_{\b S_{i_q}}} \b x_{q}^{\mathbf{v}^{i_q}_{k}(t)^{\perp}} \bm{1}_{q k}(t), \\
\frac{\partial f_{p}}{\partial \gamma_{k}}(t) &=\frac{1}{\sqrt{m}} \frac{c_{k}}{\left\|\mathbf{v}_{k}(t)\right\|_{\b S_{i_p}}} \sigma\left(\mathbf{v}_{k}(t)^{\top} \mathbf{x}_{p}\right),  \\
\frac{\partial L}{\partial \gamma_{k}}(t) &=\frac{1}{\sqrt{m}} \sum_{q=1}^{N M}\left(f_{q}(t)-y_{q}\right) \frac{c_{k}}{\left\|\mathbf{v}_{k}(t)\right\|_{\b S_{i_q}}} \sigma\left(\mathbf{v}_{k}(t)^{\top} \mathbf{x}_{q}\right),
\end{aligned}
\end{align*}
where $f_p = f(\b x^{i_p}_p)$, $\b x_{p}^{\mathbf{v}^{i_p}_{k}(t)^{\perp}} \triangleq (\b I - \frac{\b S_{i_p} \b u \b{u}^\top }{\parallel \b u \parallel_{\b S_{i_p}}^2})\b x$, and $\bm{1}_{pk}(t) \triangleq \bm{1}_{\{\b v_k(t)^\top \b x_p \geq 0 \}}.$

We define Gram matrix $\b V(t)$ and $\b G(t)$ as
\begin{align}
\mathbf{V}_{p q}(t) & = 
\frac{1}{m} \sum_{k=1}^{m}\left(\alpha c_{k} \cdot \gamma_{k}(t)\right)^2 \left\|\mathbf{v}_{k}(t)\right\|_{\b S_{i_p}}^{-1} \left\|\mathbf{v}_{k}(t)\right\|_{\b S_{i_q}}^{-1} \left\langle\mathbf{x}_{p}^{\mathbf{v}^{i_p}_{k}(t)^{\perp}}, \mathbf{x}_{q}^{\mathbf{v}^{i_q}_{k}(t)^{\perp}}\right\rangle \bm{1}_{p k}(t) \bm{1}_{q k}(t), \label{equ: fedavg_v} \\
\mathbf{G}_{p q}(t) & =
\frac{1}{m} \sum_{k=1}^{m}  c_{k}^{2} \left\|\mathbf{v}_{k}(t)\right\|_{\b S_{i_p}}^{-1} \left\|\mathbf{v}_{k}(t)\right\|_{\b S_{i_q}}^{-1}  \sigma\left(\mathbf{v}_{k}(t)^{\top} \mathbf{x}_{p}\right) \sigma\left(\mathbf{v}_{k}(t)^{\top} \mathbf{x}_{q}\right). \label{equ: fedavg_g_apdx}
\end{align}
It follows that
\begin{align*}
T_{\mathbf{v}}^{p}(t)=\sum_{q=1}^{N M} \frac{\mathbf{V}_{p q}(t)}{\alpha^{2}}\left(f_{q}(t)-y_{q}\right), \quad
T_{\mathbf{\gamma}}^{p}(t)=\sum_{q=1}^{N M} \mathbf{G}_{p q}(t)\left(f_{q}(t)-y_{q}\right).
\end{align*}
Let $\mathbf{f}=\left(f_{1}, \ldots, f_{n}\right)^{\top}=\left(f\left(\mathbf{x}_{1}\right), \ldots, f\left(\mathbf{x}_{NM}\right)\right)^{\top}$. The full evolution dynamic is given by
\begin{align*}
\frac{d \mathbf{f}}{d t}=-\boldsymbol{\Lambda}(t)(\mathbf{f}(t)- \b y), \quad \text{where} \quad
\boldsymbol{\Lambda}(t):=\frac{\mathbf{V}(t)}{\alpha^{2}}+\mathbf{G}(t).
\end{align*}


Similarly, we compute Gram matrix $\b V^*(t)$ and $\b G^*(t)$ for FedBN with $f^*$ as
\begin{align}
\mathbf{V}^*_{p q}(t) &= 
\frac{1}{m} \sum_{k=1}^{m}\left(\alpha c_{k} \right)^2 \gamma_{k,i_p}(t) \gamma_{k,i_q}(t) \left\|\mathbf{v}_{k}(t)\right\|_{\b S_{i_p}}^{-1} \left\|\mathbf{v}_{k}(t)\right\|_{\b S_{i_q}}^{-1} \left\langle\mathbf{x}_{p}^{\mathbf{v}^{i_p}_{k}(t)^{\perp}}, \mathbf{x}_{q}^{\mathbf{v}^{i_q}_{k}(t)^{\perp}}\right\rangle \bm{1}_{p k}(t) \bm{1}_{q k}(t), \label{equ: fedbn_v} \\
\mathbf{G}^*_{p q}(t) & =\frac{1}{m} \sum_{k=1}^{m}  c_{k}^{2} \left\|\mathbf{v}_{k}(t)\right\|_{\b S_{i_p}}^{-1} \left\|\mathbf{v}_{k}(t)\right\|_{\b S_{i_q}}^{-1}  \sigma\left(\mathbf{v}_{k}(t)^{\top} \mathbf{x}_{p}\right) \sigma\left(\mathbf{v}_{k}(t)^{\top} \mathbf{x}_{q}\right) \bm{1}\{i_p = i_q\}. \label{equ: fedbn_g_apdx} 
\end{align}
Thus, the full evolution dynamic of FedBN is
\begin{align*}
\frac{d \mathbf{f}^*}{d t}=-\boldsymbol{\Lambda}^*(t)(\mathbf{f}^*(t)- \b y), \quad \text{where} \quad
\boldsymbol{\Lambda}^*(t):=\frac{\mathbf{V}^*(t)}{\alpha^{2}}+\mathbf{G}^*(t).
\end{align*}

\subsection{Proof of Lemma \ref{lemma:eigen}}
\label{sec:proof_lemma}
\cite{dukler2020optimization} proved that the matrix $\b G^{\infty}$ is strictly positive definite. In their proof, $\b G^{\infty}$ is the covariance matrix of the functionals $\phi_p$ define as
\[
\phi_{p}(\b v) := \sigma \left( \mathbf{v}^{\top} \mathbf{x}_{p} \right) 
\]
over the Hilbert space $\mathcal{V}$ of $L^{2}\left(N\left(0, \alpha^{2} \mathbf{I}\right)\right)$. $\b G^{*\infty}$ is strictly positive definite by showing that $\phi_1,\cdots,\phi_{NM}$ are linearly independent, which is equivalent to that 
\begin{align}
\label{equ: inde_phi}
c_{1} \phi_{1}+c_{2} \phi_{2}+\cdots+c_{NM} \phi_{NM}=0 \text{ in } \mathcal{V}
\end{align}
holds only for $c_p=0$ for all $p$.

Let $\b G^{\infty}_i$ denote the $i$-th $M \times M$ block matrices on the diagonal of $\b G^{\infty}$. Then we have
\begin{align*}
    \b G^{*\infty} = diag(\b G^{\infty}_1,\cdots,\b G^{\infty}_N).
\end{align*}
To prove that $\b G^{*\infty}$ is strictly positive definite, we will show that $\b G^{\infty}_i$ is positive definite. Let us define 
\[
\phi^*_{j,i}(\b v) := \sigma \left( \mathbf{v}^{\top} \mathbf{x}_{j} \right) \bm{1}\{j \in \text{ site } i \}, \quad j=1,\cdots, M.
\]
Then, we are going to show that
\begin{align}
\label{equ: inde_phi2}
c_{1} \phi^*_{1,i}+c_{2} \phi^*_{2,i}+\cdots+c_{M} \phi^*_{M,i}=0 
\end{align}
holds only for $c_j=0, \forall j \in [M]$. Suppose there exist
$c_{1},\cdots,c_{M}$ that are not identically 0, satisfying (\ref{equ: inde_phi2}). Let the coefficients for client $i$ be $c_{1},\cdots,c_{M}$ and let the coefficients for other client
be 0. Then, we have a sequence of coefficients satisfying (\ref{equ: inde_phi}), which is a contradiction with that $\b G^{\infty}$ is strictly positive definite. This implies $\b G^{\infty}_i$ is strictly positive definite. Namely, $\b G^{\infty}_i$'s eigenvalues are positive.  Since the eigenvalues of $\b G^{*\infty}$ are exactly the union of the eigenvalues of $\b G^{\infty}_i$, $\lambda_{min}(\b G^{*\infty})$ is positive and thus, $\b G^{*\infty}$ is strictly positive definite.

\subsection{Proof of Corollary \ref{coro:comp}}

To compare the convergence rates of FedAvg and FedBN when $E=1$, we compare the exponential factor in the convergence rates, which are $\left(1-\eta \mu_{0}/2\right)$ and $\left(1-\eta \mu^*_{0}/2\right)$ for FedAvg and FedBN, respectively.
 Then, it reduces to comparing $\mu_{0} = \lambda_{\min}(\b G^{\infty})$ and $\mu^*_0 = \lambda_{\min}(\b G^{*\infty})$. 
 Comparing equation (\ref{equ: fedavg_g_apdx}) and (\ref{equ: fedbn_g_apdx}), $\b G^{*\infty}$ takes the $M \times M$ block matrices on the diagonal of $\b G^{\infty}$:
 \[
\b G^{\infty}=\left[\begin{array}{cccc}
\b G^{\infty}_1 & \b G^{\infty}_{1,2}  & \cdots & \b G^{\infty}_{1,N}  \\
\b G^{\infty}_{1,2} & \b G^{\infty}_2 & \cdots & \b G^{\infty}_{2,N}  \\
\vdots & \vdots & \ddots & \vdots \\
\b G^{\infty}_{1,N} &\b G^{\infty}_{2,N} & \cdots & \b G^{\infty}_N
\end{array}\right], \quad
\b G^{*\infty}=\left[\begin{array}{cccc}
\b G^{\infty}_{1} & 0 & \cdots & 0 \\
0 & \b G^{\infty}_{2} & \cdots & 0 \\
\vdots & \vdots & \ddots & \vdots \\
0 & 0 & \cdots &\b G^{\infty}_{N}
\end{array}\right],
 \]
where $\b G^{\infty}_i$ is the $i$-th $M \times M$ block matrices on the diagonal of $\b G^{\infty}$. By linear algebra, 
\[
\lambda_{\min}(\b G^{\infty}_i) \geq \lambda_{\min}(\b G^{\infty}), \quad  \forall i \in [N].
\]
 Since the eigenvalues of $\b G^{*\infty}$ are exactly the union of eigenvalues of $\b G^{\infty}_i$, we have 
 \begin{align*}
 \lambda_{\min}(\b G^{*\infty}) & = \min_{i \in [N]} \{ \lambda_{\min}(\b G^{\infty}_i) \}, \\
 & \geq \lambda_{\min}(\b G^{\infty}).
 \end{align*}
% \Xiaoxiao{Xiaofei, we may need to write as $\lambda_{\min}(\b G^{*\infty})  \geq \min(\lambda_{\min}(\b G^{\infty}_i))$}\\
Thus, $\left(1-\eta \mu_{0}/2\right) \geq \left(1-\eta \mu^*_{0}/2\right)$ and we can conclude that the convergence rate of FedBN is faster than the convergence of FedAvg.


==> future.tex <==
\section{Discussion and Future Work}

\Xiaoxiao{This is a first draft for the discussion. It is far from good. Your comments are very welcome!}

In classical federated learning, a new client can be added to a system by initializing this client with the current global parameters. In FedBN, however, the BN parameters are not shared. This issue can be overcome by sharing BN parameters as well and initializing a new client with the average BN parameters. We detail this approach in Appendix~\ref{app:test}.

FedBN is independent of the optimization strategy, communication scheme, and the aggregation technique. Thus, it can be used with various optimizers~\citep{}, efficient communication schemes (e.g., averaging random subsets~\citep{mcmahan2017communication}, dynamic averaging~\citep{kamp2019black}),%, or compression~\citep{suresh2017distributed}),
and aggregation techniques (e.g., geometric median~\citep{pillutla2019robust}, Radon machines~\citep{kamp2017effective}, or distributed distillation~\citep{bistritz2020distributed}).

Since batch normalization is often applied in multiple layers within a network architecture, normalization affects different representations of the data and thus allows for a more complex normalization than usual forms of data preprocessing. Thus, we believe that FedBN improves a wide range of applications, most prominently autonomous driving and healthcare. In both cases, local clients might capture data using different sensors or equipment (sensor types vary between vehicle types or generations, in hospitals the imaging equipment can vary). An interesting direction for future work is analyzing what types of differences in local data can be ironed out by FedBN and where the limits of the method lie. Moreover, not sharing local BN parameters should make inference on local data more challenging. It would be interesting to quantify this improvement in privacy.

\begin{enumerate}
    \item Privacy
    \item Healthcare
    \item Methods (whether BN can be replaced with other normalization)
    \item Aggregate BN using clustering. 
    \item Contact MONAI and Clara
    \item Camera Ready -- 1. Future work: the methods can be intergrated with other optimization strategy such as FedAdam, aggregating strategies.  2. Put a table with combination results. 3. Proof-reading the manuscript. 
    \item Add out of domain client case in discussion session but do not include the table.
    \item Add ``sharing BN parameters will cause higher communication costs and privacy issues'' to some where.
\end{enumerate}

==> illustration.tex <==





